The California Legacy Survey I. A Catalog of 178 Planets from Precision Radial Velocity Monitoring of 719 Nearby Stars over Three Decades

We present a high-precision radial velocity (RV) survey of 719 FGKM stars, which host 164 known exoplanets and 14 newly discovered or revised exoplanets and substellar companions. This catalog updated the orbital parameters of known exoplanets and long-period candidates, some of which have decades-longer observational baselines than they did upon initial detection. The newly discovered exoplanets range from warm sub-Neptunes and super-Earths to cold gas giants. We present the catalog sample selection criteria, as well as over 100,000 radial velocity measurements, which come from the Keck-HIRES, APF-Levy, and Lick-Hamilton spectrographs. We introduce the new RV search pipeline RVSearch that we used to generate our planet catalog, and we make it available to the public as an open-source Python package. This paper is the first study in a planned series that will measure exoplanet occurrence rates and compare exoplanet populations, including studies of giant planet occurrence beyond the water ice line, and eccentricity distributions to explore giant planet formation pathways. We have made public all radial velocities and associated data that we use in this catalog.

==> planet_citations.tex <==
145675: Wittenmyer07, Butler03
1461: Rivera10
1461: Diaz16
155358: Robertson12
155358: Stassun17
69830: Lovis06
69830: Lovis06
69830: Lovis06
102195: Ge06
104067: Segransan11
10697: Butler06
107148: Butler06
108874: Butler03
108874: Vogt05
114729: Butler03
114762: Butler06
114783: Vogt02
114783: Bryan16
115617: Vogt10
115617: Vogt10
115617: Vogt10
117176: Naef04
117207: Marcy05
120136: Butler97
12661: Fischer01
12661: Butler06
126614: Howard10
128311: Butler03
128311: Vogt05
130322: Udry00
134987: Butler01
134987: Jones10
13931: Howard10
141399: Vogt14
141399: Vogt14
141399: Vogt14
141399: Vogt14
143761: Noyes97
143761: Fulton16
145934: Feng15
154345: Wright08
156279: Diaz12
156279: Bryan16
156668: Howard11
16141: Butler06
164922: Butler06
164922: Fulton16
167042: Johnson08
168443: Wittenmyer07
168443: Wittenmyer07
168746: Pepe02
169830: Naef01
169830: Mayor04
170469: Fischer07
177830: Butler06
177830: Meschiari11 (Suspect)
179949: Tiney01
183263: Marcy05
183263: Wright09
186427: Chochran97
187123: Vogt00
187123: Wright09
188015: Marcy05
190360: Naef03
190360: Vogt05
192263: Santos00
192310: Howard11(b?)
192310: Pepe11 (Miss this one, activity mucks it up)
195019: Fischer99
209458: Charbonneau00 & Henry00
210277: Marcy99
217014: Mayor95
217107: Vogt05
217107: Vogt05
218566: Meschiari11
219134: Vogt15
219134: Vogt15
219134: Vogt15
219134: Vogt15
219134: Vogt15
22049: Hatzes00
222582: Vogt00
24040: Boisse12
32963: Rowan16
33636: Vogt02
34445: Howard10
34445: Vogt17 
34445: Vogt17 
34445: Vogt17 (miss a few of their candidates)
3651: Butler06
38529: Fischer01
38529: Butler06
40979: Butler06
4203: Vogt02
4203: Kane14
4208: Vogt02
42618: Fulton16
45184: Udry19
45184: Udry19
45350: Marcy05
46375: Marcy00
49674: Butler03
50499: Vogt05
50499: Rickman19
50554: Fischer02
52265: Butler00
66428: Butler06
72659: Butler03
74156: Naef04
74156: Naef04
75732: Butler97
75732: McArthur04
75732: Marcy02
75732: McArthur04
75732: Fischer08
7924: Fulton15
7924: Fulton15
7924: Fulton15
82943: Mayor04
82943: Mayor04
8574: Perrier03
87883: Fischer09
92788: Fischer01
92788: Rickman19
9446: Hebrard10
9446: Hebrard10
95128: Naef04
95128: Wittenmyer07
95735: Diaz19
97658: Howard11
9826: Butler97
9826: Naef04
9826: Naef04
99109: Butler06
99492: Marcy05
175541: Johnson07
181234: Rickman19
11964a: Butler06
11964a: Wright09
gj3470: Bonfils12
gl317: Johnson07b
gl317: Anglada-Escude12
gl687: Burt14
hip109388: Butler06_GJ849
hip109388: Feng15
hip22627: Howard10
hip57050: Haghighipour10
hip57050: Trifonov17
hip74995: Bonfils05
hip83043: Johnson10
bd-103166: Butler00
37124: Butler03
37124: Butler03
37124: Vogt05
68988: Vogt02
80606: Wittenmyer07
120066: Blunt19
1326: Howard14
